Building Affordance Relations for Robotic Agents - A Review

Affordances describe the possibilities for an agent to perform actions with an object. While the significance of the affordance concept has been previously studied from varied perspectives, such as psychology and cognitive science, these approaches are not always sufficient to enable direct transfer, in the sense of implementations, to artificial intelligence (AI)-based systems and robotics. However, many efforts have been made to pragmatically employ the concept of affordances, as it represents great potential for AI agents to effectively bridge perception to action. In this survey, we review and find common ground amongst different strategies that use the concept of affordances within robotic tasks, and build on these methods to provide guidance for including affordances as a mechanism to improve autonomy. To this end, we outline common design choices for building representations of affordance relations, and their implications on the generalisation capabilities of an agent when facing previously unseen scenarios. Finally, we identify and discuss a range of interesting research directions involving affordances that have the potential to improve the capabilities of an AI agent.

==> sections/5_future_directions.tex <==
\section{Discussion on Future Directions \label{sec:challenges}}
    
    We have explored the different approaches in the literature for including affordances in various robotics tasks. The different design choices (Section~\ref{sc:design_choices}), and learning time of the affordance relation (Section~\ref{sc:deployment}), determine the method's ability to generalise to previously unseen scenarios.
    Given this diversity and the fact that is a relatively new research area, affordances in robotics offer interesting opportunities for researchers to contribute to the progress and maturity of the field. The objective of this section is to outline possible areas of contribution based on the study of the reviewed literature.
    
    %----------------------------------- 
    \subsection{Design choices and their influence \label{ssc:summary}}
        As previously mentioned, the choices of data input and learning time influence, differently, the performance of the methods. Nonetheless, some design choices have been explored more than others, thus leaving room for research with regards to the generalisation capabilities that can be achieved. Fig.~\ref{fig:coverage} shows a coverage map of the reviewed literature spread over the different design choices. The warmer the colour, the more used the strategy is across the literature. For example, most of the work emphasises the learning of primitive actions as affordances (i.e., push, grasp, lift among others), using visual perception and image labels from images to get an affordance per target object, building the affordance relation probabilistically. 
        On the opposite side, colder coloured elements, indicate there are very few approaches that exploit learning affordance trajectories in the form of motions (using kinaesthetic sensing), as well as those that exploit a multi-step prediction to achieve the tasks in a planning manner. Certainly, some of these components are highly dependent on hardware robustness more than others. Nonetheless, studying such aspects in greater depth would improve their inclusion in robotics tasks as well as provide valuable insights for collaboration activities and task replication across different agents.
    
        % \clearpage
         \begin{figure}[t!]
            \centering
              \includegraphics[width=8.9cm]{figures/population.pdf}
           
            \caption{Population map, from the reviewed literature, of the design choices of work that includes affordances in their robotic tasks. The warmer the colour (red) the more the work uses that element to design their affordance relation model, while the colder the colour (green), the less that element is used.}
            \label{fig:coverage}
        \end{figure}
       
    %-------------------------------------
    \subsection{Data acquisition and processing correlation \label{sec:challenges_is}}
        Given that the field requires different types of data, (i.e., target object, action and effects), there is an inherent need to cross-correlate data structures. These associations can be further enriched by diversifying data acquisition and processing. For example, knowing that a cup in a kitchen is likely to afford pouring liquid while in a bathroom might also serve as a toothbrush holder requires the agent to be able to relate not only object features but also the surroundings. Moreover, the data acquisition should not be limited to visual object features but, instead, it should account for the object's material, texture and other physical properties to enhance the agent's interaction with the object. By using such cross-correlation, the affordance relation models could provide the agents with the ability to generalise affordances as associations of objects' visual and physical characteristics, as well as with the surrounding context.
     
    %-------------------------------------
    \subsection{Autonomous behaviour learning \label{sec:challenges_ma}}
        At present, the idea of including the concept of affordances in robotic applications has centred on performing one robotic task at the time. Most of the work either detects one object affordance, such as a glass affords pouring, but rarely proceeds to perform the pouring task. The field would benefit from a methodology that is able to unify associations of target objects with a library of actions and an online evaluation of the effects. This association would allow the agent to obtain feedback on the performance of the task and rectify it online. Such a method would open doors to autonomously concatenate goal-oriented tasks (e.g., preparing a recipe, cleaning dishes), explore the feasibility of subsequent motion controllers and the interpretability of natural language instructions for largely scaled tasks. 
    
   

==> sections/table_datasets.tex <==
% what if we shorten the URL (e.g. [link here]), and include more relevant info, such as year, ...?
% should we sort them?

\begin{table*}[ht!]
    \caption{Available affordance datasets for robotics. Datasets location clickable with paper online version.% All the actions considered in these datasets are identified as complex actions. %\textcolor{red}{double check this \url{https://arxiv.org/pdf/1807.06775.pdf}} 
    \label{tb:datasets}}

    \centering
    \begin{tabular}{p{3.1cm}|p{2.5cm}|p{3cm}|p{3.5cm}|p{3.5cm}}
    \hline
    \multicolumn{1}{c|}{\textbf{Work}} & \multicolumn{1}{c|}{\textbf{Task}} & \multicolumn{1}{c|}{\textbf{Contains}} & \multicolumn{1}{c|}{\textbf{Type of Data}} & \multicolumn{1}{c}{\textbf{Dataset Location}} \\ \hline
  
    \mbox{\cite{ardon2019learning}} & Manipulation & 30 objects / 7 scenes / 14 actions & RGB-D images, 3D models / 3D poses, image labels / semantic relations & \url{https://paolaardon.github.io/grasp_affordance_reasoning/} \\ \hline
    
    \mbox{\cite{castellini2011using}} & Manipulation & 7 objects / 5 actions & RGB images / 3D poses, image labels &
    \url{http://www.slipguru.unige.it/Data/VMGdB/} \\ \hline
    
    \cite{chu2019learning} &Manipulation& 10 objects / 7 actions & RGB images / image labels & \url{https://dropbox.com/s/ldapcpanzqdu7tc/models.zip} \\ \hline
    
    \mbox{\cite{dehban2016moderately}} & Manipulation & 14 objects / 4 actions & RGB images / image labels &\url{https://github.com/vislab-tecnico-lisboa/affordance-datasets} \\ \hline
    
    \cite{jiang2013hallucinated} & Object \& Action Recognition & 47 objects / 4 scenes / 6 human poses associated with actions & RGB-D images, 3D models / 3D poses, image labels & \url{http://pr.cs.cornell.edu/hallucinatinghumans/}  \\\hline
    
    \mbox{\cite{koppula2016anticipatory}} & Object \& Action Recognition & 10 human poses associated with actions & RGB-D images, 3D models / 3D poses, image labels & \url{http://pr.cs.cornell.edu/humanactivities/} \\ \hline
    
    \cite{myers2015affordance} & Manipulation& 105 tool-handles / 3 scenes / 7 actions & RGB-D images / image labels & \url{http://users.umiacs.umd.edu/~fer/affordance/} \\ \hline
    
    \cite{nguyen2017object} & Object Recognition & 10 objects / 9 actions & RGB images / image labels & \url{https://sites.google.com/site/ocnncrf/} \\ \hline
    
    \mbox{\cite{sawatzky2017weakly}} & Object Recognition & 12 objects / 6 actions & RGB-D images, 3D models / 3D poses, image labels & \url{https://zenodo.org/record/495570#.XyBkBZNKhlc} \\ \hline
    
    \cite{shu2016learning} & Action Prediction &  human poses associated with 5 actions & RBG-D images / 3D poses &
    \url{https://www.tshu.io/SocialAffordance/} \\ \hline
    
    \cite{thermos2017deep} & Manipulation & 14 objects/ 13 actions& RGB-D images / 3D poses&
    \url{http://sor3d.vcl.iti.gr/} \\ \hline
    
    \cite{varadarajan2012afrob} & Manipulation & 25 geometries / 10 materials / 33 actions  & RGB-D images / image labels / semantic relations & \url{http://www.theaffordances.net/} \\ \hline

    \cite{zhu2015understanding} & Object Recognition & 19 objects / 3 actions & RGB-D images, 3D models / 3D poses, image labels & \url{https://yzhu.io/publication/tool2015cvpr/} \\ \hline
    
    \end{tabular}
\end{table*}
